RubCSG at SemEval-2022 Task 5: Ensemble learning for identifying misogynous MEMEs

This work presents an ensemble system based on various uni-modal and bi-modal model architectures developed for the SemEval 2022 Task 5: MAMI-Multimedia Automatic Misogyny Identification. The challenge organizers provide an English meme dataset to develop and train systems for identifying and classifying misogynous memes. More precisely, the competition is separated into two sub-tasks: sub-task A asks for a binary decision as to whether a meme expresses misogyny, while sub-task B is to classify misogynous memes into the potentially overlapping sub-categories of stereotype, shaming, objectification, and violence. For our submission, we implement a new model fusion network and employ an ensemble learning approach for better performance. With this structure, we achieve a 0.755 macroaverage F1-score (11th) in sub-task A and a 0.709 weighted-average F1-score (10th) in sub-task B.

==> Sections/delete.tex <==
\subsection{Graph convolutional network}\label{GCNapp}



\subsection{Example combining the OCR and image caption text}\label{textcomb}



\subsection{Force teaching weighted binary cross-entropy loss }\label{weightloss}

In weighted binary cross-entropy loss, the weights are obtained by:
\begin{equation} \label{lossweight}
    w_{\textrm{loss}_{i}} = \frac{\frac{\textrm{NoS}}{\textrm{NoS}(i)}}{\sum_{j}^{}\frac{\textrm{NoS}}{\textrm{NoS}(j)}}, i \in [\textrm{Shm}, \textrm{Str}, \textrm{Obj}, \textrm{Vio}]
\end{equation}

where $\textrm{NoS}$ is the total number of samples in the training set. $\textrm{NoS}(i)$ represents the number of true instances for class $i$. Only four categories are considered in sub-task B: shaming, stereotype, objectification, and violence. Finally, the multi-label loss value is computed through the weighted combination of the binary cross-entropy:
\begin{equation} \label{loss}
\textrm{loss}1 = \sum_{i}^{}w_{\textrm{loss}_{i}}\cdot \textrm{BCE}(p_i, \textrm{target}_i).
\end{equation}
$p_i$ is the probability of class $i$ and $\textrm{target}_i$ is the ground truth. 

Due to the relationship between sub-task A and B, we adopted force teaching in the loss function for better performance. The sample should be first identified as misogynous and then classified into four categories. So, we add a force teaching term:


\begin{equation} \label{mse}
\textrm{loss}2 = \textrm{MSE}(\textrm{pseudo}_{_\textrm{Mis}}, \textrm{target}_{_\textrm{Mis}}), 
\end{equation}
where
\begin{equation} \label{mse1}
\textrm{pseudo}_{_\textrm{Mis}} = \textrm{max}(p_{_\textrm{Shm}}, p_{_\textrm{Ste}}, p_{_\textrm{Obj}}, p_{_\textrm{Vio}}).
\end{equation}
The final loss is computed by
\begin{equation} \label{lossend}
\textrm{loss} = 0.7\times \textrm{loss}1 + 0.3 \times \textrm{loss}2.
\end{equation}


\subsection{\emph{Setup-A} results for sub-task A}\label{sub-taska}

Sub-task A focuses on misogynous memes identification. Three single-modal models are first trained. Based on the single-modal models, the multi-modal models BERTC-Vit, GCAN-Vit, BERTC-GCAN, and BERTC-GCAN-Vit are optimized through our proposed fusion network (Figure~\ref{fig:mmms}). Figure~\ref{fig:subtaskacv} uses the Mann-Whitney-U test~\cite{mann1947test} to indicate statistically significant differences in the F1-score between the BERTC model and other models for sub-task A. 

\begin{figure}[h]
        \centering
        \includegraphics[scale=0.5]{./Sections/Image/subtaska1.pdf}
         \caption{Sub-task A macro-average F1-score for 10-fold cross validation. Asterisks indicate a statistically significant
difference, where *** denotes 1e-04 < p <= 1e-03, * denotes 1e-02 < p <= 5e-02, ns denotes p > 5e-02.}
         \label{fig:subtaskacv}
\end{figure}


\begin{table}[H]
\setlength{\tabcolsep}{3pt} % Default value: 6pt

\begin{tabular}{|c|c|c|c|}
\hline
model     & ensemble & model          & ensemble \\ \hline
BERTC     & 0.663            & GCAN-Vit                                                  & \textbf{0.707}            \\ \hline
GCAN      & 0.674            & BERTC-GCAN                                                & 0.677            \\ \hline
Vit       & 0.619            & \begin{tabular}[c]{@{}c@{}}BERTC-\\ GCAN-Vit\end{tabular} & 0.689            \\ \hline
BERTC-Vit & 0.697            & -                                                         & -                \\ \hline
\end{tabular}
\caption{Soft voting ensemble performance with \emph{setup-A} for sub-task A}
\label{subtaskacv}
\end{table}

Table~\ref{subtaskacv} lists the model soft voting ensemble F1-score in 10-fold cross-validation. The GCAN-Vit model still outperforms other models after the soft voting ensemble. Finally, the model-level hard voting ensemble is adopted and yields 0.698 F1-score. %However, our models for sub-task A suffered from overfitting on the official test set. In the early research stage, we worked only on the training set with 10,000 samples. 700 samples were randomly selected and split from the training set as a temp test set. The rest 9,300 samples were used as the training set to train our proposed models, 10-fold cross-validation was still applied. Our ensemble results on the temp test set were over 0.87. It could be due to a higher level of similarity between the training set and the temp test set.

\subsection{Significance comparison for \emph{setup-B}  results}\label{sub-taskb}
%\vspace{-0.2cm}
\begin{figure}[!htb]
        \centering
       \includegraphics[scale=0.5]{./Sections/Image/subtaskb1.pdf}
         \caption{Sub-task A model performance significance comparison}
         \label{sigA}
\end{figure}

Figure~\ref{sigA} gives the sub-task A results, computed from \emph{setup-B}. Figure~\ref{sigB} is the results of sub-task B.  Again, the multi-modal model GCAN-Vit outperforms other models.


\begin{figure}[!htb]
        \centering
       \includegraphics[scale=0.5]{./Sections/Image/subtaskb2.pdf}
         \caption{Sub-task B model performance significance comparison}
         \label{sigB}
\end{figure}

